Yelp Reviews and Food Types: A Comparative Analysis of Ratings, Sentiments, and Topics

This study examines the relationship between Yelp reviews and food types, investigating how ratings, sentiments, and topics vary across different types of food. Specifically, we analyze how ratings and sentiments of reviews vary across food types, cluster food types based on ratings and sentiments, infer review topics using machine learning models, and compare topic distributions among different food types. Our analyses reveal that some food types have similar ratings, sentiments, and topics distributions, while others have distinct patterns. We identify four clusters of food types based on ratings and sentiments and find that reviewers tend to focus on different topics when reviewing certain food types. These findings have important implications for understanding user behavior and cultural influence on digital media platforms and promoting cross-cultural understanding and appreciation.

==> citation.tex <==
@inproceedings{sara2017authenticity,
  title={Authenticity in Online Ethnic Restaurant Reviews: Revealing Conflicted Nationalism in Multicultural Consumption},
  author={Sara, K},
  booktitle={Annual Meeting of the Agriculture, Food, and Human Values Society and the Association for the Study of Food and Society},
  year={2017}
}

@article{li2020racism,
  title={Racism in tourism reviews},
  author={Li, Shu and Li, Gang and Law, Rob and Paradies, Yin},
  journal={Tourism Management},
  volume={80},
  pages={104100},
  year={2020},
  publisher={Elsevier}
}

@article{chen2013investigation,
  title={An investigation into online reviewers' behavior},
  author={Chen, Hua-Ning and Huang, Chun-Yao},
  journal={European Journal of Marketing},
  volume={47},
  number={10},
  pages={1758--1773},
  year={2013},
  publisher={Emerald Group Publishing Limited}
}

@article{zukin2017omnivore,
  title={The omnivore’s neighborhood? Online restaurant reviews, race, and gentrification},
  author={Zukin, Sharon and Lindeman, Scarlett and Hurson, Laurie},
  journal={Journal of Consumer Culture},
  volume={17},
  number={3},
  pages={459--479},
  year={2017},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{nakayama2019cultural,
  title={The cultural impact on social commerce: A sentiment analysis on Yelp ethnic restaurant reviews},
  author={Nakayama, Makoto and Wan, Yun},
  journal={Information \& Management},
  volume={56},
  number={2},
  pages={271--279},
  year={2019},
  publisher={Elsevier}
}

@phdthesis{choi2021empirical,
  title={An empirical study identifying bias in Yelp dataset},
  author={Choi, Seri and others},
  year={2021},
  school={Massachusetts Institute of Technology}
}

@article{tong2021evaluation,
  title={Evaluation of online consumer reviews of hospitals and experiences of racism using qualitative methods},
  author={Tong, Jason and Andy, Anietie U and Merchant, Raina M and Kelz, Rachel R},
  journal={JAMA Network Open},
  volume={4},
  number={9},
  pages={e2126118--e2126118},
  year={2021},
  publisher={American Medical Association}
}

@article{boch2021mainstream,
  title={Mainstream flavor: Ethnic cuisine and assimilation in the United States},
  author={Boch, Anna and Jim{\'e}nez, Tom{\'a}s and Roesler, Katharina},
  journal={Social Currents},
  volume={8},
  number={1},
  pages={64--85},
  year={2021},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{le2021exploring,
  title={Exploring the multi-dimensionality of authenticity in dining experiences using online reviews},
  author={Le, Truc H and Arcodia, Charles and Novais, Margarida Abreu and Kralj, Anna and Phan, Thanh Cong},
  journal={Tourism Management},
  volume={85},
  pages={104292},
  year={2021},
  publisher={Elsevier}
}

@article{yu2023food,
  title={Food “taste” on Yelp: displays of cultural omnivorousness and authenticity in dining choices and online reviews},
  author={Yu, Chao and Margolin, Drew},
  journal={Food, Culture \& Society},
  volume={26},
  number={1},
  pages={3--23},
  year={2023},
  publisher={Taylor \& Francis}
}

@article{labelle2022pandemic,
  title={Pandemic-Induced Anti-Asian Sentiment in Chicago: An Exploratory Analysis of Restaurant Yelp Reviews},
  author={LaBelle-Hahn, Alana},
  year={2022},
  publisher={University of Chicago}
}

@inproceedings{quan2022implicit,
  title={Implicit Discriminatory Bias Reflected in Yelp Reviews-A case study},
  author={Quan, Wei and Li, Zhijian and Kim, Wonkyung},
  booktitle={2022 IEEE International Conference on Big Data (Big Data)},
  pages={6799--6801},
  year={2022},
  organization={IEEE}
}

@inproceedings{hutto2014vader,
  title={Vader: A parsimonious rule-based model for sentiment analysis of social media text},
  author={Hutto, Clayton and Gilbert, Eric},
  booktitle={Proceedings of the international AAAI conference on web and social media},
  volume={8},
  number={1},
  pages={216--225},
  year={2014}
}

@article{ha2010perceived,
  title={Perceived values, satisfaction, and behavioral intentions: The role of familiarity in Korean restaurants},
  author={Ha, Jooyeon and Jang, SooCheong Shawn},
  journal={International Journal of Hospitality Management},
  volume={29},
  number={1},
  pages={2--13},
  year={2010},
  publisher={Elsevier}
}

@article{jeong2011restaurant,
  title={Restaurant experiences triggering positive electronic word-of-mouth (eWOM) motivations},
  author={Jeong, EunHa and Jang, SooCheong Shawn},
  journal={International Journal of Hospitality Management},
  volume={30},
  number={2},
  pages={356--366},
  year={2011},
  publisher={Elsevier}
}

@article{ryu2012influence,
  title={The influence of the quality of the physical environment, food, and service on restaurant image, customer perceived value, customer satisfaction, and behavioral intentions},
  author={Ryu, Kisang and Lee, Hye-Rin and Kim, Woo Gon},
  journal={International journal of contemporary hospitality management},
  volume={24},
  number={2},
  pages={200--223},
  year={2012},
  publisher={Emerald Group Publishing Limited}
}

@article{SajnaniYelp,
  title={Multilabel Classification of Reviews in Yelp Data},
  author={H. Sajnani, and V. Saini, and K. Kumar, and E. Gabrielova, and P. Choudary, and C. Lopes},
  journal={Technical report},
  year={2014}
}

@article{loper2002nltk,
  title={Nltk: The natural language toolkit},
  author={Loper, Edward and Bird, Steven},
  journal={arXiv preprint cs/0205028},
  year={2002}
}

==> resources/citation.tex <==
@inproceedings{sara2017authenticity,
  title={Authenticity in Online Ethnic Restaurant Reviews: Revealing Conflicted Nationalism in Multicultural Consumption},
  author={Sara, K},
  booktitle={Annual Meeting of the Agriculture, Food, and Human Values Society and the Association for the Study of Food and Society},
  year={2017}
}

@article{li2020racism,
  title={Racism in tourism reviews},
  author={Li, Shu and Li, Gang and Law, Rob and Paradies, Yin},
  journal={Tourism Management},
  volume={80},
  pages={104100},
  year={2020},
  publisher={Elsevier}
}

@article{chen2013investigation,
  title={An investigation into online reviewers' behavior},
  author={Chen, Hua-Ning and Huang, Chun-Yao},
  journal={European Journal of Marketing},
  volume={47},
  number={10},
  pages={1758--1773},
  year={2013},
  publisher={Emerald Group Publishing Limited}
}

@article{zukin2017omnivore,
  title={The omnivore’s neighborhood? Online restaurant reviews, race, and gentrification},
  author={Zukin, Sharon and Lindeman, Scarlett and Hurson, Laurie},
  journal={Journal of Consumer Culture},
  volume={17},
  number={3},
  pages={459--479},
  year={2017},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{nakayama2019cultural,
  title={The cultural impact on social commerce: A sentiment analysis on Yelp ethnic restaurant reviews},
  author={Nakayama, Makoto and Wan, Yun},
  journal={Information \& Management},
  volume={56},
  number={2},
  pages={271--279},
  year={2019},
  publisher={Elsevier}
}

@phdthesis{choi2021empirical,
  title={An empirical study identifying bias in Yelp dataset},
  author={Choi, Seri and others},
  year={2021},
  school={Massachusetts Institute of Technology}
}

@article{tong2021evaluation,
  title={Evaluation of online consumer reviews of hospitals and experiences of racism using qualitative methods},
  author={Tong, Jason and Andy, Anietie U and Merchant, Raina M and Kelz, Rachel R},
  journal={JAMA Network Open},
  volume={4},
  number={9},
  pages={e2126118--e2126118},
  year={2021},
  publisher={American Medical Association}
}

@article{boch2021mainstream,
  title={Mainstream flavor: Ethnic cuisine and assimilation in the United States},
  author={Boch, Anna and Jim{\'e}nez, Tom{\'a}s and Roesler, Katharina},
  journal={Social Currents},
  volume={8},
  number={1},
  pages={64--85},
  year={2021},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{le2021exploring,
  title={Exploring the multi-dimensionality of authenticity in dining experiences using online reviews},
  author={Le, Truc H and Arcodia, Charles and Novais, Margarida Abreu and Kralj, Anna and Phan, Thanh Cong},
  journal={Tourism Management},
  volume={85},
  pages={104292},
  year={2021},
  publisher={Elsevier}
}

@article{yu2023food,
  title={Food “taste” on Yelp: displays of cultural omnivorousness and authenticity in dining choices and online reviews},
  author={Yu, Chao and Margolin, Drew},
  journal={Food, Culture \& Society},
  volume={26},
  number={1},
  pages={3--23},
  year={2023},
  publisher={Taylor \& Francis}
}

@article{labelle2022pandemic,
  title={Pandemic-Induced Anti-Asian Sentiment in Chicago: An Exploratory Analysis of Restaurant Yelp Reviews},
  author={LaBelle-Hahn, Alana},
  year={2022},
  publisher={University of Chicago}
}

@inproceedings{quan2022implicit,
  title={Implicit Discriminatory Bias Reflected in Yelp Reviews-A case study},
  author={Quan, Wei and Li, Zhijian and Kim, Wonkyung},
  booktitle={2022 IEEE International Conference on Big Data (Big Data)},
  pages={6799--6801},
  year={2022},
  organization={IEEE}
}

@inproceedings{hutto2014vader,
  title={Vader: A parsimonious rule-based model for sentiment analysis of social media text},
  author={Hutto, Clayton and Gilbert, Eric},
  booktitle={Proceedings of the international AAAI conference on web and social media},
  volume={8},
  number={1},
  pages={216--225},
  year={2014}
}

@article{ha2010perceived,
  title={Perceived values, satisfaction, and behavioral intentions: The role of familiarity in Korean restaurants},
  author={Ha, Jooyeon and Jang, SooCheong Shawn},
  journal={International Journal of Hospitality Management},
  volume={29},
  number={1},
  pages={2--13},
  year={2010},
  publisher={Elsevier}
}

@article{jeong2011restaurant,
  title={Restaurant experiences triggering positive electronic word-of-mouth (eWOM) motivations},
  author={Jeong, EunHa and Jang, SooCheong Shawn},
  journal={International Journal of Hospitality Management},
  volume={30},
  number={2},
  pages={356--366},
  year={2011},
  publisher={Elsevier}
}

@article{ryu2012influence,
  title={The influence of the quality of the physical environment, food, and service on restaurant image, customer perceived value, customer satisfaction, and behavioral intentions},
  author={Ryu, Kisang and Lee, Hye-Rin and Kim, Woo Gon},
  journal={International journal of contemporary hospitality management},
  volume={24},
  number={2},
  pages={200--223},
  year={2012},
  publisher={Emerald Group Publishing Limited}
}

@article{SajnaniYelp,
  title={Multilabel Classification of Reviews in Yelp Data},
  author={H. Sajnani, and V. Saini, and K. Kumar, and E. Gabrielova, and P. Choudary, and C. Lopes},
  journal={Technical report},
  year={2014}
}

@article{loper2002nltk,
  title={Nltk: The natural language toolkit},
  author={Loper, Edward and Bird, Steven},
  journal={arXiv preprint cs/0205028},
  year={2002}
}
